TransFG: A Transformer Architecture for Fine-grained Recognition

Fine-grained visual classification (FGVC) which aims at recognizing objects from subcategories is a very challenging task due to the inherently subtle inter-class differences. Most existing works mainly tackle this problem by reusing the backbone network to extract features of detected discriminative regions. However, this strategy inevitably complicates the pipeline and pushes the proposed regions to contain most parts of the objects thus fails to locate the really important parts. Recently, vision transformer (ViT) shows its strong performance in the traditional classification task. The self-attention mechanism of the transformer links every patch token to the classification token. In this work, we first evaluate the effectiveness of the ViT framework in the fine-grained recognition setting. Then motivated by the strength of the attention link can be intuitively considered as an indicator of the importance of tokens, we further propose a novel Part Selection Module that can be applied to most of the transformer architectures where we integrate all raw attention weights of the transformer into an attention map for guiding the network to effectively and accurately select discriminative image patches and compute their relations. A contrastive loss is applied to enlarge the distance between feature representations of confusing classes. We name the augmented transformer-based model TransFG and demonstrate the value of it by conducting experiments on five popular fine-grained benchmarks where we achieve state-of-the-art performance. Qualitative results are presented for better understanding of our model.

==> 07_rebuttal.tex <==
\newcommand{\ROne}{\textcolor{orange}{\textbf{R1}}}
\newcommand{\RTwo}{\textcolor{purple}{\textbf{R2}}}
\newcommand{\RThree}{\textcolor{cyan}{\textbf{R3}}}

\section{Rebuttal-TransFG: A Transformer Architecture for Fine-Grained Recognition}

We thank all three reviewers for their insightful comments. We make our best effort to answer all critical questions in detail. We will make a very thorough update of the paper draft regarding the suggestions.

\centering \textbf{Response to Reviewer1}

\begin{enumerate}
    \item \textbf{Novelty}. Our main novelty lies in the idea of exploiting the selected parts and this helps to reveal why Vision Transformer performs generally better in the context of fine-grained recognition from one perspective. This is to say that though the technique of aggregating attention weights from different transformer layers does come from (Abnar and Zuidema 2020) and we do not make big modifications to it except removing the re-normalization step on attention weights. We interestingly find that by only exploiting the selected most important tokens is enough for the model to make high-precision recognition. This phenomenon offers a novel interpretation of Vision Transformer as a part-based model. As revealed by the ViT paper, Vision Transformer has a relatively large receptive field even at early layers so it naturally establish spatial relations between tokens. And as it goes deeper, the global connections between tokens become stronger especially for those important ones. Thus by integrating the attention weights of different layers, we select such important parts and exploit them for successful classification. By contrast, CNN mainly exploits the local properties of images and can only capture weak global relation in very high convolution layers which makes it less suitable in the context of fine-grained recognition.
    
    \item \textbf{Effectiveness}. Actually, as can be observed on the leaderboard of many datasets in FGVC (CUB, Cars, Dogs), the performance starts to saturate and improvements by even $0.5-1.0\%$ are very significant. This is probably because these datasets are relatively small in size and as the capability of vision models increases, they are becoming somehow easy now as a benchmark. Under such situation, we achieve 1.3\%, 2.0\%, 1.6\% performance gain on CUB, Dogs, NABirds respectively which is a huge improvement. Besides, it is true that our improvements on large-scale datasets are more obvious, additional experiments on iNat18 and iNat21 shows an improvement of 2.8\% and 3.5\% respectively.
    
    \item \textbf{Justification}. Due to the page limit, we are sorry that we can not show additional qualitative examples here. But we do conduct such experiments and the conclusion is that the overall attention maps still look fine but for the most important tokens (regarding to the 1st and 3rd rows of Fig 5) the results do not match to meaningful parts precisely. This results correspond to the findings in (Abnar and Zuidema 2020). We will add this interesting experiment in the revised version.
\end{enumerate}

\centering \textbf{Response to Reviewer2}

\begin{enumerate}
    \item \textbf{Novelty}. Yes, we agree that it is natural to extend Vision Transformer to the FGVC area. But it is not straightforward to use attention weights to select tokens and expect that by only exploiting these few selected tokens we can get improvements based on ViT. The contribution and impact of this work does not limit to verifying the effectiveness of Vision Transformer architecture in FGVC but more in exploring the mechanism behind ViT. We offers a new viewpoint of the interpretation of Vision Transformer which is quite novel and it is supported by our results both quantitatively and qualitatively. For detailed discussion on this point please refer to the first point of response to Reviewer1.
    
    \item \textbf{Effectiveness}. Yes, the overlap patch split does work. It brings constant improvement on all datasets while some are relatively small, but others are more significant (e.g. 0.5\% on NABirds and 0.8\% on iNat2017). Also as discussed in the second point to the response to Reviewer1, the performance on CUB is quite saturated so it is not easy to make even small improvement. The effectiveness of the overlap split is larger than the data itself seems like. We think the reason behind the effectiveness of overlap split is that it brings back the locality which is lost in the origin ViT and offers more possible choices of tokens which correspond to discriminative parts. This will lead to a more accurate token selection and thus improve the final classification accuracy. 
\end{enumerate}

\centering \textbf{Response to Reviewer3}

\begin{enumerate}
    \item \textbf{Reasons behind Part Selection Module.} As revealed by (Abnar and Zuidema 2020) and (Sofia and Noah 2019), the raw attention weights of transformers gradually become more uniform when the layer goes deeper which makes it less relevant to the corresponding input patches. We found the similar phenomenon here in Vision Transformer as well. Thus, though the raw attention weights of the last layer do somehow capture the important parts, it is weaker when compared to the aggregation of all attention weights. Besides, it has less corresponding relationship to the origin image patches which makes it less interpretable. As a result, it is necessary to have the part selection module to integrate raw attention weights and select import parts. 
    
    As regarding to the overlap split, we think the reason of its effectiveness is that it brings back the locality which is lost in the origin ViT and offers more possible choices of tokens which correspond to discriminative parts. This will further improve the accuracy of token selection which can not simply be offset by the global view of vision transformer.
    
    \item \textbf{Part Selection Module as regularization.} It is interesting to view Part Selection Module as a regularization besides its original effect as discussed in the paper. We also think that the success of it lies in filtering out less relevant tokens before the last step which is similar to the idea of regularization. Current experiments show that we can get constant improvement on both large-scale or small datasets (the size of many fine-grained datasets are already quite small especially for Vision Transformers). But it would be definitely interesting to see what the situation will be with even fewer data. We will carefully design the experiments and add it to the revised version.
\end{enumerate}
